One Network to Solve Them All --- Solving Linear Inverse Problems using Deep Projection Models

While deep learning methods have achieved state-of-the-art performance in many challenging inverse problems like image inpainting and super-resolution, they invariably involve problem-specific training of the networks. Under this approach, different problems require different networks. In scenarios where we need to solve a wide variety of problems, e.g., on a mobile camera, it is inefficient and costly to use these specially-trained networks. On the other hand, traditional methods using signal priors can be used in all linear inverse problems but often have worse performance on challenging tasks. In this work, we provide a middle ground between the two kinds of methods --- we propose a general framework to train a single deep neural network that solves arbitrary linear inverse problems. The proposed network acts as a proximal operator for an optimization algorithm and projects non-image signals onto the set of natural images defined by the decision boundary of a classifier. In our experiments, the proposed framework demonstrates superior performance over traditional methods using a wavelet sparsity prior and achieves comparable performance of specially-trained networks on tasks including compressive sensing and pixel-wise inpainting.

==> arxiv_imgnet_figures.tex <==





\def\dataset{imgnet}
\def\denoise{denoise_ratio0.50_std0.10}
\def\denoiseours{ours_alpha0.300000}
\def\denoisel{l1_lambdal10.100000_alpha0.300000}
\def\cs{cs_ratio0.10_std0.00}
\def\csours{ours_alpha0.300000}
\def\csl{l1_lambdal10.030000_alpha0.300000}
\def\inpaint{inpaint_bs6_tb10_std0.00}
\def\inpaintours{ours_alpha0.050000}
\def\inpaintl{l1_lambdal10.030000_alpha0.300000}
\def\inpaintc{inpaintcenter_bs19_std0.00}
\def\inpaintcours{ours_alpha0.300000}
\def\inpaintcl{l1_lambdal10.030000_alpha0.300000}
\def\superres{superres_ratio0.50_std0.00}
\def\superresours{ours_alpha0.500000}
\def\superresl{l1_lambdal10.030000_alpha0.500000}
\def\special{speical}












\begin{figure*}[t]
	\centering
	% first row %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\def\idxone{905}
	\def\idxtwo{222}
	\def\idxthree{8013}
	\def\idxfour{804}
	\def\idxfive{603}
	\def\idxsix{18793}
	\def\idxseven{9783}
	\def\idxeight{12345}
	\def\idxnine{15213}
	\def\idxten{230}
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cblankcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Ccscol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cdenoisecol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cinpaintcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cblockcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Csuperrescol}
		\end{subfigure}	
			\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Ccscol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cdenoisecol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cinpaintcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cblockcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Csuperrescol}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Ccscol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cdenoisecol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cinpaintcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Cblockcol}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\caption*{\Csuperrescol}
		\end{subfigure}	
	\end{subfigure}
	\\
	%%%%%%%%%%%%%%%%%%  intputs
	\vspace{\sixteenimgrowmargin}
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\groundtruthrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/ori_img.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/y.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxone/\superres/y.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxtwo/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxthree/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}	
	\\
	%%% our results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\vspace{3mm}
			\caption*{\oursrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csours/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoiseours/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresours/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% l1 results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\vspace{3mm}
			\caption*{\lrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csl/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoisel/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresl/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% specialized results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\srowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\special/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\special/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\special/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% second big row
%%%%%%%%%%%%%%%%%%  intputs
	\def\idxone{\idxfour}
	\def\idxtwo{\idxfive}
	\def\idxthree{\idxsix}
	\vspace{\sixteenimgrowmargin}
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\groundtruthrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/ori_img.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/y.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxone/\superres/y.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxtwo/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxthree/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}	
	\\
	%%% our results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\vspace{3mm}
			\caption*{\oursrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csours/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoiseours/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresours/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% l1 results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\vspace{3mm}
			\caption*{\lrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csl/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoisel/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresl/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% specialized results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\srowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\special/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\special/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\special/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%% third big row
	%%%%%%%%%%%%%%%%%%  intputs
	\def\idxone{\idxseven}
	\def\idxtwo{\idxeight}
	\def\idxthree{\idxnine}
	\vspace{\sixteenimgrowmargin}
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\groundtruthrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/ori_img.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/y.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/y.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxone/\superres/y.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxtwo/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/ori_img.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/y.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/y.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{-0.75\textwidth}
			\includegraphics[width=0.5\textwidth]{figures/\dataset/\idxthree/\superres/y.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}	
	\\
	%%% our results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{3mm}
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\oursrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csours/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoiseours/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcours/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresours/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csours/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoiseours/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcours/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresours/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% l1 results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\vspace{3mm}
			\caption*{\lrowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\csl/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\denoisel/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\inpaintl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\inpaintcl/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\superresl/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\csl/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\denoisel/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\inpaintl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\inpaintcl/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\superresl/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	%%% specialized results
	\begin{subfigure}{\linewidth}
		\centering
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\vspace{\sixteenimgrowcaptionheight}
			\caption*{\srowcaption}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\cs/\special/z.jpg}
			%			\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\denoise/\special/z.jpg}
			%			\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaint}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxone}/{\inpaintc}/\special/z.jpg}
			%			\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxone/\superres/\special/z.jpg}
			%			\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx2
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxtwo}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxtwo/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
		\hspace{0.5mm}
		%%%%%% idx3
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\cs/\special/z.jpg}
			%		\caption*{\Cori}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\denoise/\special/z.jpg}
			%		\caption*{\Cdenoise}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaint}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}	
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/{\dataset}/{\idxthree}/{\inpaintc}/\special/z.jpg}
			%		\caption*{\Cinpaint}
		\end{subfigure}
		\begin{subfigure}[t]{\sixteenimgwidth}
			\centering
			\includegraphics[width=\textwidth]{figures/\dataset/\idxthree/\superres/\special/z.jpg}
			%		\caption*{\Csuperres}
		\end{subfigure}	
	\end{subfigure}
	\vspace{-3mm}
	\caption{\small Results on ImageNet dataset. PSNR values are shown at the lower-right corners. Compressive sensing uses $\frac{m}{d} = 0.1$.  For pixelwise inpainting, we drop $50\%$ of the pixels and add Gaussian noise with $\sigma=0.1$.  We use $\rho=0.05$ on blockwise inpainting and $\rho=0.5$ on super resolution.  }
	\label{figure: imgnet}
\end{figure*}

































